Large Language Models as Data Preprocessors

Large Language Models (LLMs), typified by OpenAI's GPT, have marked a significant advancement in artificial intelligence. Trained on vast amounts of text data, LLMs are capable of understanding and generating human-like text across a diverse range of topics. This study expands on the applications of LLMs, exploring their potential in data preprocessing, a critical stage in data mining and analytics applications. Aiming at tabular data, we delve into the applicability of state-of-the-art LLMs such as GPT-4 and GPT-4o for a series of preprocessing tasks, including error detection, data imputation, schema matching, and entity matching. Alongside showcasing the inherent capabilities of LLMs, we highlight their limitations, particularly in terms of computational expense and inefficiency. We propose an LLM-based framework for data preprocessing, which integrates cutting-edge prompt engineering techniques, coupled with traditional methods like contextualization and feature selection, to improve the performance and efficiency of these models. The effectiveness of LLMs in data preprocessing is evaluated through an experimental study spanning a variety of public datasets. GPT-4 emerged as a standout, achieving 100\% accuracy or F1 score on 4 of these datasets, suggesting LLMs' immense potential in these tasks. Despite certain limitations, our study underscores the promise of LLMs in this domain and anticipates future developments to overcome current hurdles.

==> concl.tex <==
\section{Conclusion and Future Work}
\label{sec:concl}
% We investigated the case of using three SOTA LLMs, GPT-3.5, GPT-4, and Vicuna 
% for four data preprocessing tasks. We discussed the strengths and limitations 
% of LLMs in these tasks. Following recent advancements in understanding and 
% utilizing LLMs, we designed prompts for the four tasks which integrate 
% techniques such as impersonation, zero- and few-shot prompting, and batch 
% prompting. We performed an experimental evaluation on a set of widely-used 
% datasets. The results demonstrated the superiority of the evaluated LLMs, 
% especially GPT4, in data imputation, schema matching, and entity matching, and 
% justified the usefulness of our prompting techniques. As a preliminary study 
% on using LLMs for data preprocessing, we expect that future works will center 
% around addressing the limitations in domain specification, nonsensical output, 
% efficiency, etc. 
We investigated the application of SOTA LLMs for four data preprocessing tasks. We assessed the 
strengths and identified the limitations of these LLMs for the aforementioned 
tasks. Drawing on recent advancements in understanding and leveraging LLMs, we 
crafted prompts and integrated prompting techniques. An empirical evaluation 
was conducted on a selection of widely-used datasets. The results showcased the 
superiority of the evaluated LLMs, particularly GPT-4 in data preprocessing. 
These results substantiate the effectiveness of our prompting techniques. 
%As a preliminary study on utilizing LLMs for data preprocessing, 
We anticipate that future research will focus on addressing the discussed 
limitations. 
% concerning domain specification, nonsensical output, efficiency, and other related issues.

==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{VLDB Workshop Reference Format:}\\
\vldbauthors. \vldbtitle. VLDB \vldbyear\ Workshop: \vldbworkshop.\\ %\vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
%\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment. %, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
%\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
% \ifdefempty{\vldbavailabilityurl}{}{
% \vspace{.3cm}
% \begingroup\small\noindent\raggedright\textbf{VLDB Workshop Artifact Availability:}\\
% The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
% \endgroup
% }
%%% VLDB block end %%%

==> vldbinfo.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbyear{2024}
% name of the workshop
\newcommand\vldbworkshop{Tabular Data Analysis Workshop (TaDA)}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{URL_TO_YOUR_ARTIFACTS}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{empty} 

